Calculus for the Modern Engineer: Putting the Joy Back in Learning Advanced Mathematics

Many engineering students enter college excited about math and physics, only to have their enthusiasm dimmed by a rigid, outdated calculus curriculum. The University of Michigan's Robotics Department is piloting a new 4-credit course, ``Calculus for the Modern Engineer,'' to reintroduce the excitement of learning advanced mathematics. Integrating Differential and Integral Calculus, vector derivatives, and Ordinary Differential Equations (ODEs) into a unified one-semester curriculum, the course emphasizes conceptual mastery and real-world applications. It starts with definite integration -- building on students' intuitive understanding of sums -- before progressing through limits, differentiation, antiderivatives, and ODEs. By leveraging computational tools like Julia, Large Language Models (LLMs), and Wolfram Alpha Pro, it reduces reliance on tedious hand calculations. Case studies in numerical integration, optimization, and feedback control connect theory to engineering challenges. Supported by an open-source textbook and programming assignments, the course equips students with modern computational skills and reignites their passion for mathematics.

==> Defines/definesJuliaCodeCell.tex <==
%\usepackage{listingsutf8}

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{listings}


\usepackage{xcolor}

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.98,0.92,0.97}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}

%%
%% Julia definition (c) 2014 Jubobs
%%
\lstdefinelanguage{Julia}%
  {morekeywords={abstract,break,case,catch,const,continue,do,else,elseif,%
      end,export,false,for,function,immutable,import,importall,if,in,%
      macro,module,otherwise,quote,return,switch,true,try,type,typealias,%
      using,while},%
   sensitive=true,%
   alsoother={$},%
   morecomment=[l]\#,%
   morecomment=[n]{\#=}{=\#},%
   morestring=[s]{"""}{"""},%
   morestring=[m]{"}{"},%
}[keywords,comments,strings]%

\lstdefinestyle{mystyle}{
frame=tb,
  language=Julia,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle=\ttfamily,
  backgroundcolor=\color{backcolour},
  numberstyle=\tiny{\bf \color{black}},
  keywordstyle={\bf \color{blue}},
  commentstyle=\color{dkgreen},
  identifierstyle={\bf \color{black}},
  stringstyle=\color{mauve},
  breakatwhitespace=false,         
  breaklines=true,                 
  captionpos=b,                    
  keepspaces=true,                 
  numbers=left,                    
  numbersep=5pt,                  
  showspaces=false,                
  showstringspaces=false,
  showtabs=false,                  
  tabsize=2
}

\lstset{style=mystyle}

    % commentstyle=\itshape\color{purple!40!black},
    % identifierstyle=\color{blue},
    % backgroundcolor=\color{gray!10!white}

==> Sections/ROB101andROB201Content.tex <==
\section{ROB 101 Contents Overview}

\textsmc{ROB 101 Computational Linear Algebra} is structured to introduce first-year students to computational linear algebra as a foundational tool for robotics and engineering. Its chapters are organized as follows:

\begin{enumerate}

\item {\bf Introduction to Systems of Linear Equations}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 2 hours lecture + recitation.
    \item Students are introduced to foundational algebraic concepts to build intuition for systems of equations.
    \item Examples are used to explore unique, no, and infinite solutions.
    \item Includes a brief programming exercise to introduce basic matrix operations in Julia.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Recognize and classify systems of linear equations by their possible solutions;
    \item Develop a basic understanding of solution methods, including substitution and elimination;
    \item Appreciate that these hand-methods do not scale;
    \item Build familiarity with the role of systems of equations in robotics and engineering applications.
\end{inparaenum}

\textbf{Content:} Linear equations with unique solutions, no solutions, and infinite solutions; solving systems via substitution and elimination; interpreting solutions graphically; introduction to $Ax = b$ as a unifying framework for systems of linear equations. (Optional Reads: Historical development of linear equations, relevance in robotics and autonomous systems.)

\vspace*{.1cm}

\item {\bf Vectors, Matrices, and Determinants}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 4 hours lecture + recitation.
    \item Introduces matrix representation and operations for systems of equations.
    \item Focus on the determinant as a key property of matrices.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand vectors and matrices as special forms of arrays that provide a convenient ``database'' for expressing linear systems of equations. At this point, vectors and matrices are not yet mathematical objects. 
    \item Explore the properties of determinants and their applications;
    \item Represent and solve systems of equations in matrix form.
\end{inparaenum}

\textbf{Content:} Definition of vectors and matrices, operations with matrices, introduction to determinants, and their role in determining the solvability of systems of equations. (Optional Reads: Additional properties of determinants.)

\vspace*{.1cm}

\item {\bf Triangular Systems of Equations: Forward and Back Substitution}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 4 hours lecture + recitation.
    \item Demonstrates solving triangular systems as a simplified case of linear systems.
    \item Students implement forward and back substitution in Julia.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Solve lower and upper triangular systems of equations;
    \item Develop computational methods for substitution;
    \item Determinants can be computed by inspection for triangular matrices; 
    \item Understand the significance of triangular matrices in numerical methods.
\end{inparaenum}

\textbf{Content:} Forward substitution, back substitution, lower and upper triangular matrices, applications in computational linear algebra. (Optional Reads: Numerical stability in triangular systems.)

\vspace*{.1cm}

\item {\bf Matrix Multiplication}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 3 hours lecture + recitation.
    \item Covers the mechanics and significance of matrix multiplication.
    \item Applications include transformations and compositions.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Perform standard matrix multiplication;
    \item Understand the relationship between rows and columns in matrix operations;
    \item Learn the outer-product formulation of matrix multiplication, setting students up for an easy way to perform LU factorization; 
    \item Apply matrix multiplication to practical problems.
\end{inparaenum}

\textbf{Content:} Row and column views of matrix multiplication, examples, and applications in robotics transformations. (Optional Reads: Proof for the alternative outer-product formulation of matrix multiplication.)

\vspace*{.1cm}

\item {\bf LU (Lower-Upper) Factorization}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 3 hours lecture + recitation.
    \item Focuses on breaking systems into triangular components for easier computation;
    \item Students implement LU factorization in Julia, without pivoting; 
    \item Examples where pivoting is essential are explained and illustrated with Julia's built-in tools.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand the concept of LU factorization;
    \item Solve systems of equations using LU decomposition;
    \item Relate LU factorization to triangular systems.
\end{inparaenum}

\textbf{Content:} LU factorization, solving $Ax = b$ using LU, and applications in numerical computation. (Optional Reads: Algorithms for LU with pivoting.)

\vspace*{.1cm}

\item {\bf Determinants, Matrix Inverses, and Transposes}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 2 hours lecture + recitation.
    \item Explores essential matrix properties and their implications for linear systems.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Compute determinants and inverses of matrices;
    \item Apply the concept of matrix transpose;
    \item Recognize the significance of these properties in solving equations.
\end{inparaenum}

\textbf{Content:} Determinants, inverse matrices, properties of transposes, and practical computation methods. (Optional Reads: Advanced matrix identities.)

\vspace*{.1cm}

\item {\bf The Vector Space $\mathbb{R}^n$: Part 1}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 4 hours lecture + recitation.
    \item Introduces students to the abstract properties of vector spaces.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Define and understand vector spaces;
    \item Analyze linear independence and span;
    \item Relate vector spaces to solutions of $Ax = b$.
\end{inparaenum}

\textbf{Content:} Definition of vector spaces, linear independence, span, and applications in robotics. (Optional Reads: Basis and dimension.)

\vspace*{.1cm}

\item {\bf Norms and Least-Squares Solutions}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 3 hours lecture + recitation.
    \item Introduces optimization concepts through least-squares methods.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Compute norms and interpret their significance;
    \item Apply least-squares methods to solve overdetermined systems;
    \item Explore regression as a practical application.
\end{inparaenum}

\textbf{Content:} Vector norms, least-squares solutions, regression, and applications. (Optional Reads: Generalized least-squares methods.)

\vspace*{.1cm}

\item {\bf The Vector Space $\mathbb{R}^n$: Part 2}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 5 hours lecture + recitation.
    \item Explores orthogonality and its applications in linear algebra.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand orthogonal vectors and matrices;
    \item Apply the Gram-Schmidt process;
    \item Explore QR factorization.
\end{inparaenum}

\textbf{Content:} Orthogonality, Gram-Schmidt process, QR factorization, and practical applications. (Optional Reads: Modified Gram-Schmidt.)

\vspace*{.1cm}

\item {\bf Eigenvalues, Eigenvectors, and Advanced Concepts}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 3 hours lecture + recitation.
    \item Introduces eigenvalues and eigenvectors.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Compute eigenvalues and eigenvectors;
    \item Understand their role in linear transformations;
    \item Apply these concepts in robotics and dynamics.
\end{inparaenum}

\textbf{Content:} Eigenvalues, eigenvectors, diagonalization, and applications. (Optional Reads: Spectral theorem.)

\vspace*{.1cm}

\item {\bf Solutions of Nonlinear Equations}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 3 hours lecture + recitation.
    \item Introduces methods for solving nonlinear systems;
    \item Main point is to show how linear approximations of nonlinear functions allow techniques from linear algebra to be applied to a much broader class of problems.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Introduce numerical differentiation and linear approximations of nonlinear functions;
    \item Explore numerical methods for nonlinear equations;
    \item Apply Newton-Raphson method;
    \item Understand Jacobians and gradients through numerical differentiation, primarily, central or symmetric differences.
\end{inparaenum}

\textbf{Content:} Bisection, Newton-Raphson, Jacobians, and gradients. (Optional Reads: Applications in robotics, such a calibration of a LiDAR sensor.)

\vspace*{.1cm}

\item {\bf Basics of Optimization}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 4 hours lecture + recitation.
    \item Introduces optimization methods in robotics.
\end{inparaenum}



\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Apply gradient descent;
    \item Understand the role of the Hessian matrix;
    \item Solve constrained and unconstrained optimization problems using tools in Julia.
\end{inparaenum}

\textbf{Content:} Gradient descent, Hessians, optimization in robotics. (Optional Reads: Quadratic programming.)

\vspace*{.1cm}

\item {\bf Background for Machine Learning}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 2 hours lecture + recitation.
    \item Provides foundational concepts for machine learning.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand separating hyperplanes and classifiers;
    \item Understand signed-distance;
    \item Apply max-margin classifiers;
    \item Explore orthogonal projections.
\end{inparaenum}

\textbf{Content:} Separating hyperplanes, max-margin classifiers, orthogonal projection, and applications. (Optional Reads: Soft-margin classifiers.)
    
\end{enumerate}

\subsection{Three Pillar Projects in ROB 101}

ROB 101 bridges the gap between theoretical linear algebra and its applications through three cornerstone projects, each designed to highlight the real-world relevance of matrix mathematics. These projects immerse students in practical problem-solving, computational implementation, and a taste of robotics and intelligent systems.

\textbf{Building 3D Maps from LiDAR Data:} The first project, focusing on computer vision and mapping, introduces students to the processing of LiDAR data. Through this project, students learn to generate and manipulate point clouds, a foundational concept in robotics and autonomous systems. Using tools in Julia, they transform raw LiDAR scans into structured maps, gaining hands-on experience with matrix transformations and 3D visualizations. This project not only reinforces linear algebra concepts but also shows how these tools power technologies such as autonomous vehicles and drones.

\textbf{Regression of Large Data Sets:} The second project shifts attention to machine learning and climate data analysis. Here, students work with real-world climate datasets to apply regression techniques based on least-squares optimization. By exploring the mathematical underpinnings of these methods, students discover the power of linear algebra in making predictions and uncovering patterns in large datasets. This project serves as a gateway to understanding the role of data-driven decision-making in engineering and science, laying the groundwork for advanced study in machine learning and artificial intelligence.

\textbf{Stabilizing a Simple Model of a Segway via MPC:} The third and final project is a capstone experience that challenges students to design a feedback control system for a Segway. Students begin by modeling the dynamics of a Segway, applying concepts of state-variable representation and discrete dynamics. They then use model predictive control (MPC) techniques, framed as underdetermined least-squares optimization problems, to develop a controller capable of balancing and stabilizing the system. This project culminates in the implementation of the control algorithm in Julia, providing students with a tangible understanding of how mathematics, coding, and engineering come together to solve complex problems.

Through these projects, students not only deepen their understanding of linear algebra but also experience the excitement of applying mathematical theory to modern engineering challenges. Each project is carefully designed to inspire curiosity, build confidence, and provide a glimpse into the possibilities awaiting them in robotics and intelligent systems.

\newpage

\section{ROB 201 Contents Overview}


The textbook accompanying \textsc{Calculus for the Modern Engineer} is a comprehensive resource, covering everything from basic pre-calculus principles to advanced topics like ODEs, Laplace transforms, and proportional-derivative feedback controllers. The book places equal weight on the conceptual and computational sides of calculus. Concepts are first grounded in intuition, followed by epsilon-delta arguments and limits as needed, and are always closely followed by computations in Julia that illustrate the ideas and implement the associated formulas.

The material begins with a review of notation, functions, and algebraic manipulation before diving into the heart of calculus: definite integration. After covering the Riemann integral, the text explores differentiation, symbolic computation, and practical applications such as optimization with constraints. Students learn to use tools like SymPy and Wolfram Alpha Pro to perform symbolic manipulations, and they apply these concepts to robotics case studies involving mobile robots. The textbook concludes with chapters on improper integrals, ordinary differential equations, and Laplace transforms, the latter framed through the lens of feedback control and modern robotics applications.

\begin{enumerate}

\item {\bf Pre-calculus: Notation, Functions, and Various Algebraic Facts}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 2-hour lecture.
    \item Students are expected to review this material mostly on their own. 
    \item 20-question quiz to ensure mastery.
    \item The Approximation Principle is highlighted in HW01.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Recognize the utility of mathematical notation for precision and expressivity;
    \item Understand and apply the Bisection Algorithm as an example of the Approximation Principle;
    \item Reaffirm understanding of fundamental concepts such as functions, domains, ranges, and inverses.
\end{inparaenum}

\textbf{Content:} Introduction, Got Calculus Dread? Additional Resources, Notation or the Language of Mathematics, The Approximation Principle, Algebraic Manipulation and Inequalities, Functions (Domains, Ranges, Inverses, and Compositions), Trigonometric and Inverse Trigonometric Functions, Powers and Roots, Exponentials and Logarithms, Euler’s Formula, Hyperbolic Trigonometric Functions, Summing Symbol, Binomial Theorem, Special Functions, Shifting and Scaling, and Feedback Control. (Optional Reads: Binomial Theorem meets Euler and Proofs Associated with the Chapter.)

\item {\bf Calculus Foundations: Proofs, Finite Sums, Limits at Infinity, and Geometric Sums}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 4 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand the significance of mathematical proofs;
    \item Master proof by induction and apply it to sums of powers of integers;
    \item Comprehend limits and their initial uses in calculus, with emphasis on limits at infinity for rational functions and exponentials.
\end{inparaenum}

\textbf{Content:} Introduction, Mathematical Proofs, Countable Sets, Proofs by Induction, Finite Sums, Limits at Infinity, Geometric Sums. (Optional Reads: Euler's Number, Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Definite Integration as the Signed Area Under a Curve}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 5 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Define and explain definite integration \`a la Riemann-Darboux;
    \item Execute computations using methods like Trapezoidal Rule and Simpson's Rule;
    \item Recognize applications of definite integrals in engineering.
\end{inparaenum}

\textbf{Content:} The Riemann Integral, Properties of the Riemann Integral, Numerical Methods for Approximating Integrals, Applications of Definite Integral. (Optional Reads: Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Properties of Functions: Left and Right Limits, Types of Continuity, Boundedness, and Generalizations of Max and Min}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 5 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Analyze function behavior using one-sided limits;
    \item Understand the nature of function continuity;
    \item When can limits be taken inside a function;
    \item Explore generalizations of maximum and minimum values.
\end{inparaenum}

\textbf{Content:} Limits from the Left and Right, Continuity, Maximum and Minimum Values, The Squeeze Theorem, Piecewise Continuity, Boundedness, Generalizations of Max/Min. (Optional Reads: Intermediate Value Theorem, Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Differentiation}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 5 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand single-variable and partial derivatives;
    \item Apply differentiation rules and software tools;
    \item Explore real problems where derivatives are used in engineering.
\end{inparaenum}

\textbf{Content:} Derivative as Local Slope and as Linear Approximation, Differentiation Rules, Software Tools for Computing Derivatives, Use Cases of Derivatives, Partial Derivatives, Jacobians, Gradients, Hessians, Total Derivative. (Optional Reads: Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Engineering Applications of the Derivative}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 6 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Develop strategies for solving optimization problems;
    \item Apply Lagrange’s equations to dynamics.
\end{inparaenum}

\textbf{Content:} Path Length, Root Finding, Unconstrained Minimization, Gradient Descent with and without Equality Constraints, Lagrange Multipliers, Dynamics à la Lagrange. (Optional Reads: More on Lagrangian Dynamics, Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Antiderivatives and the Fundamental Theorems of Calculus}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 5 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand antiderivatives and their relationship to definite integrals;
    \item Apply key techniques for finding antiderivatives.
\end{inparaenum}

\textbf{Content:} Introduction, Fundamental Theorems of Calculus, Antiderivatives, Techniques for Finding Antiderivatives, Software Tools for Antiderivatives. (Optional Reads: Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Improper Integrals}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 2 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Define and understand improper integrals;
    \item Explore practical applications in probability theory.
\end{inparaenum}

\textbf{Content:} Type-I Improper Integrals, Type-II Improper Integrals, Improper Integrals in Probability. (Optional Reads: Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Ordinary Differential Equations (ODEs)}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 8 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Learn analytical and numerical methods for solving ODEs;
    \item Apply ODEs to model dynamic systems in robotics.
\end{inparaenum}

\textbf{Content:} Introduction to ODEs, Higher-Order ODEs, Vector ODEs, Linear Systems of ODEs, Numerical Solutions, Matrix Exponential, Eigenvalues and Eigenvectors. (Optional Reads: Resonance in ODEs, Proofs Associated with the Chapter.)

\vspace*{.1cm}

\item {\bf Laplace Transforms through the Lens of Feedback Control}

\textbf{Notes:}
\begin{inparaenum}[$\bullet$]
    \item 10 hours lecture + recitation.
    \item Written and Julia HWs.
\end{inparaenum}

\textbf{Learning Objectives:}
\begin{inparaenum}[$\bullet$]
    \item Understand Laplace transforms and their application in solving ODEs;
    \item Derive and apply transfer functions in feedback control systems.
\end{inparaenum}

\textbf{Content:} Laplace Transform, Solving ODEs Using Laplace, Transfer Functions, Poles and Zeros, Feedback Systems, Transient Response of Systems, Proportional and Proportional-Derivative Feedback, Pre-compensators. (Optional Reads: Impulse Function, Proofs Associated with the Chapter.)
    
\vspace*{.1cm}


\end{enumerate}


The structure of \textsc{Calculus for the Modern Engineer} is supported by three major Julia-based projects, each designed to emphasize core skills while progressively building students' computational and theoretical knowledge. These projects are carefully aligned with the needs of robotics and engineering, providing students with hands-on experience that bridges mathematical concepts with real-world applications. Each project introduces students to key tools and methodologies used in modern engineering, ensuring they are equipped to tackle complex problems using both analytical and computational approaches. There are eight homework assignments where more basic skills are acquired and honed. Each assignment has two parts, a standard written component mirroring traditional expectations in hand computations, and a jupyter notebook written in Julia. All of this material will be open-sourced.


\subsection{Numerical Integration: Estimating Speed and Position with IMU Data}

The first project focuses on numerical integration, a fundamental concept in calculus and robotics. Students are tasked with using linear acceleration data collected from the IMU of a drone to estimate the drone’s velocity and position. Initially, they work with clean data, applying the Trapezoidal Rule to build a real-time estimate of speed and position:
$$ v(t) = v(t_0) + \int_{t_0}^t a(\tau) \, d \tau, $$
$$ p(t) = p(t_0) + \int_{t_0}^t v(\tau) \, d \tau. $$

As the project progresses, students encounter the real-world complication of acceleration bias, which affects the accuracy of the estimated speed and position. They are introduced to a one-line correction, reminiscent of the measurement step in Kalman Filtering, and are tasked with tuning the filter's gains to correct for this bias. While the project is deliberately short and approachable, it sets students up for more advanced topics, including ordinary differential equations (ODEs), by framing numerical integration as a stepping stone toward solving ODEs.

\subsection{Gradient Descent with Equality Constraints: From Basketball to Gymnastics and Diving} 

The second project takes students into the realm of optimization, beginning with a familiar scenario: calculating the initial speed and angle required for a basketball to make a successful free throw. Students explore multiple formulations of the problem. Initially, they solve a $2 \times 2$ system of linear equations to determine the initial speed ($v_x, v_y$) while fixing the time of flight. Next, they use gradient descent to minimize the squared distance from the basketball to the hoop, gradually adding complexity by introducing equality constraints that factor in time of flight and initial speed. 
This project then transitions to more complex optimization challenges, including modeling the dynamics of a simple gymnast as a floating-base representation of a bar with two point masses. Students optimize the time of flight and initial speed subject to linear constraints on the landing posture, utilizing the JuMP package to verify their results. The project culminates in an exciting optimization involving a hinged-model of a diver on a 10-meter platform, pushing students to refine their understanding of gradient descent with constraints. This progression from basketball to gymnastics, and finally to diving, demonstrates how optimization techniques are applied across diverse engineering problems.

\subsection{Modeling and Feedback Control of the BallBot}

The final project immerses students in the modeling and feedback control of a planar version of the BallBot, a simplified model of a robot that balances on a basketball using omni-directional wheels. Students begin by calculating the potential and kinetic energy of the robot's two components---the planar basketball and the torso---using Lagrange’s Method to derive the so-called "Robot Equations" of motion,
$$ D(q) \cdot \ddot{q} + C(q, \dot{q}) \cdot \dot{q} + G(q) = \Gamma. $$

Using software tools, students develop a linear state-variable model and transfer function representations of the BallBot. The project draws a direct comparison to the Segway, with the complete control design for the Segway provided in the course textbook. Following this methodology, students design, analyze, and test controllers for the linearized model of the BallBot, eventually extending their work to the full nonlinear model. The project offers a comprehensive introduction to feedback control, with all steps supported by Julia-based tools that make the process transparent, hands-on, and engaging.

